Uncertainty Weighted Actor-Critic for Offline Reinforcement Learning

Offline Reinforcement Learning promises to learn effective policies from previously-collected, static datasets without the need for exploration. However, existing Q-learning and actor-critic based off-policy RL algorithms fail when bootstrapping from out-of-distribution (OOD) actions or states. We hypothesize that a key missing ingredient from the existing methods is a proper treatment of uncertainty in the offline setting. We propose Uncertainty Weighted Actor-Critic (UWAC), an algorithm that detects OOD state-action pairs and down-weights their contribution in the training objectives accordingly. Implementation-wise, we adopt a practical and effective dropout-based uncertainty estimation method that introduces very little overhead over existing RL algorithms. Empirically, we observe that UWAC substantially improves model stability during training. In addition, UWAC out-performs existing offline RL methods on a variety of competitive tasks, and achieves significant performance gains over the state-of-the-art baseline on datasets with sparse demonstrations collected from human experts.

==> MACPdef-ams_manu.tex <==
% Definitions that require the amsmath.sty and amsthm.sty files
% Time-stamp: <07/01/15 18:05:06 miguel>

% -------------- Operators --------------

% Probability

\newcommand{\op}{\mbox{op}}
\newcommand{\Eop}{\operatorname{E}}
\newcommand{\mean}[2][]{\ensuremath{\Eop_{#1}\left\{#2\right\}}}
\newcommand{\meanop}{\operatorname{mean}}
\newcommand{\Mean}[2][]{\ensuremath{\meanop_{#1}\left\{#2\right\}}}
\newcommand{\aveop}{\Eop}
\newcommand{\ave}[2][]{\ensuremath{\aveop_{#1}\left\{#2\right\}}}
\newcommand{\varop}{\operatorname{var}}
\newcommand{\var}[2][]{\ensuremath{\varop_{#1}\left\{#2\right\}}}
\newcommand{\stdevop}{\operatorname{stdev}}
\newcommand{\stdev}[2][]{\ensuremath{\stdevop_{#1}\left\{#2\right\}}}
\newcommand{\covop}{\operatorname{cov}}
\newcommand{\cov}[2][]{\ensuremath{\covop_{#1}\left\{#2\right\}}}
\newcommand{\eff}{\operatorname{eff}}
\newcommand{\Prop}{\operatorname{P}}
\newcommand{\prob}[1]{\ensuremath{\Prop\left[#1\right]}}
\newcommand{\Volume}{\operatorname{vol}}
\newcommand{\volume}[1]{\ensuremath{\Volume\left(#1\right)}}

% Functions
\newcommand{\erf}{\operatorname{erf}}
\newcommand{\sgnop}{\operatorname{sgn}}
\newcommand{\sgn}[1]{\ensuremath{\sgnop\left(#1\right)}}

% Information theory
\newcommand{\KLop}{\operatorname{D}}
%\newcommand{\KLop}{\operatorname{KL}}
\newcommand{\KL}[2]{\KLop\left(#1\lVert#2\right)} % Kullback-Leibler divergence
\newcommand{\KLsym}[2]{\KLop\left(#1,#2\right)}   % Symmetrised KL divergence
%\newcommand{\inproduct}[2]{\left\langle#1,#2\right\rangle}  % inner product


\newcommand{\inproduct}[2]{\left\langle#1,#2\right\rangle}

% Set theory
% Are "card" and "im" the correct names in English?
\newcommand{\cardop}{\operatorname{card}}
\newcommand{\card}[1]{\ensuremath{\cardop\left(#1\right)}}
\newcommand{\im}{\operatorname{im}}
\newcommand{\vol}{\operatorname{vol}}
\newcommand{\convop}{\operatorname{conv}}
\newcommand{\conv}[1]{\ensuremath{\convop\left(#1\right)}}

% Matrices
\newcommand{\diagop}{\operatorname{diag}}
\newcommand{\diag}[1]{\ensuremath{\diagop\left(#1\right)}}
\newcommand{\cof}{\operatorname{cof}}           % Cofactor of a matrix element
\newcommand{\adj}{\operatorname{adj}}           % Adjunt matrix
\newcommand{\traceop}{\operatorname{Tr}}
\newcommand{\tr}[1]{\ensuremath{\traceop\left(#1\right)}}
\newcommand{\rankop}{\operatorname{rank}}
\newcommand{\rank}[1]{\ensuremath{\rankop\left(#1\right)}}
\newcommand{\Nullop}{\operatorname{null}}
\newcommand{\Null}[1]{\ensuremath{\Nullop\left(#1\right)}}
\newcommand{\rangeop}{\operatorname{range}}
\newcommand{\range}[1]{\ensuremath{\rangeop\left(#1\right)}}
\newcommand{\Dimop}{\operatorname{dim}}
\newcommand{\Dim}[1]{\ensuremath{\Dimop\left(#1\right)}}
\newcommand{\spanop}{\operatorname{span}}
\newcommand{\spn}[1]{\ensuremath{\spanop\left\{#1\right\}}}
\newcommand{\vectop}{\operatorname{vec}}
\newcommand{\vect}[1]{\ensuremath{\vectop\left(#1\right)}}
\newcommand{\condop}{\operatorname{cond}}
\newcommand{\cond}[1]{\ensuremath{\condop\left(#1\right)}}

% -------------- Theorem environments --------------
%\theoremstyle{plain}% default
\newtheorem{thm}{Theorem}%[section]
%\newtheorem{lem}[thm]{Lemma}
\newtheorem{lem}{Lemma}
%\newtheorem*{lemma*}{Lemma}
% \newtheorem{prop}[thm]{Proposition}
%\newtheorem*{prop*}{Proposition}
%\newtheorem{cor}[thm]{Corollary}
\newtheorem{cor}{Corollary}
\newtheorem{obs}[thm]{Observation}
%
%\theoremstyle{definition}
%\newtheorem{defn}[thm]{Definition}
\newtheorem{defn}{Definition}
\newtheorem{fact}{Fact}[thm]
%\newtheorem{assum}[thm]{Assumption}
\newtheorem{assum}{Assumption}
%\newtheorem*{defn*}{Definition}
%\newtheorem{exmp}{Example}[section]
%\newtheorem*{exmp*}{Example}
%\newtheorem{conj}{Conjecture}[section]
%\newtheorem*{conj*}{Conjecture}
%
%\theoremstyle{remark}
\newtheorem{rmk}[thm]{Remark}
%\newtheorem*{rmk*}{Remark}


%%% Local Variables:
%%% mode: plain-tex
%%% TeX-master: t
%%% End:


==> MACPdef_manu.tex <==
% Miguel A. Carreira-Perpinan's LaTeX macros.
% Time-stamp: <10/04/15 13:33:09 mcarreira-perpinan>

% Definitions that require only standard LaTeX2e things

% Letters used for matrices and vectors (boldface), for functions (roman), etc.



% \DeclareMathOperator*{\argmin}{argmin}
% \DeclareMathOperator*{\argmax}{argmax}
% \DeclareMathOperator*{\minimize}{minimize}
% \DeclareMathOperator*{\maximize}{maximize}
\newcommand{\led}[1]{\overset{\text{\ding{#1}}}{\leq}}
\newcommand{\lqq}[1]{\overset{\text{\ding{#1}}}{=}}
\newcommand{\lee}[1]{\overset{\text{\ding{#1}}}{=}}
\newcommand{\ged}[1]{\overset{\text{\ding{#1}}}{\geq}}
\newcommand{\Diag}{\text{Diag}}
\newcommand{\st}{{\text{s.t.}}}
\newcommand{\noise}{\textup{\scriptsize{noise}}}
\newcommand{\thres}{\textup{\scriptsize{thres}}}
\newcommand{\hy}[1]{\textcolor{red}{#1}}
\newcommand{\Rss}[2]{{\mathbb{R}^{#1\times#2}}}
\newcommand{\Rs}[1]{{\mathbb{R}^{#1}}}
\newcommand{\kl}{\textbf{KL}}


\newcommand{\epsi}[1]{{\epsilon_{#1}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\wmi}[1]{\bm{w}_{#1}}
\newcommand{\wmii}[1]{\bm{w}^{#1}}
\newcommand{\task}{\mathcal{T}}
\newcommand{\Ti}[1]{T_{#1}}
\newcommand{\T}{T}
\newcommand{\bi}[1]{b_{#1}}
\newcommand{\wms}{\bm{w}^{*}}
\newcommand{\wmsi}[1]{\bm{w}^{*}_{#1}}
\newcommand{\wmssi}[1]{\bm{w}^{*}_{#1,i}}
\newcommand{\wsi}[1]{\widehat{\bm{w}}^{*}_{#1}}
\newcommand{\SSi}[1]{D_{T_{#1}}}
\newcommand{\Ee}{E}
%\newcommand{\BRML}{\text{BRML}}
\newcommand{\BRML}{}
\newcommand{\phis}{\widehat{\phi}}

\newcommand{\etai}[1]{\eta_{#1}}
\newcommand{\sigmai}[1]{\sigma_{(#1)}}
\newcommand{\xmi}[1]{\bm{x}_{#1}}
\newcommand{\ymi}[1]{\bm{y}_{#1}}
\newcommand{\zmi}[1]{\bm{z}_{#1}}
\newcommand{\zmbari}[1]{\bar{\bm{z}}_{#1}}
\newcommand{\zmhati}[1]{\hat{\bm{z}}_{#1}}
\newcommand{\zmti}[1]{\widetilde{\bm{z}}_{#1}}
%\newcommand{\xmii}[2]{\bm{x}^{#1}_{#2}}
\newcommand{\ami}[1]{\bm{a}_{#1}}
\newcommand{\gmi}[1]{\bm{g}^{#1}}
\newcommand{\gti}[1]{\widetilde{\bm{g}}^{#1}}
\newcommand{\ghi}[1]{\widehat{\bm{g}}^{#1}}
\newcommand{\fii}[1]{f^{#1}}
\newcommand{\xti}[1]{\tilde{\bm{x}}^{#1}}
\newcommand{\vti}[1]{\tilde{\bm{v}}^{#1}}
\newcommand{\zmii}[2]{\bm{z}^{#1}_{#2}}
\newcommand{\zti}[2]{\widetilde{\bm{z}}^{#1}_{#2}}
\newcommand{\xmii}[2]{\bm{x}^{#1}_{#2}}
\newcommand{\dmii}[2]{\bm{\delta}^{#1}_{#2}}
\newcommand{\phii}[2]{\bm{\phi}^{#1}_{#2}}

\newcommand{\ci}[1]{c_{#1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Sb}{\bar{\mathcal{S}}}
\newcommand{\Sbi}[1]{{\bar{\mathcal{S}}}_{#1}}
\newcommand{\Sti}[1]{{\widetilde{\mathcal{S}}}_{#1}}
\newcommand{\Sm}{\mathcal{S}}
\newcommand{\proj}{\mathcal{P}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\Y}{\mathcal{Y}}
\newcommand{\LL}{\mathcal{L}}
\newcommand{\J}{\mathcal{J}}

\newcommand{\0}{\bm{0}}
\newcommand{\balpha}{\bm{\alpha}}
\newcommand{\bbeta}{\bm{\beta}}

\newcommand{\am}{\bm{a}}
\newcommand{\bmm}{\bm{b}}
\newcommand{\dm}{\bm{d}}
\newcommand{\emm}{\bm{e}}
\newcommand{\gm}{\bm{g}}
\newcommand{\wm}{\bm{\theta}}
\newcommand{\xm}{\bm{x}}
\newcommand{\ym}{\bm{y}}
\newcommand{\hmm}{\bm{h}}
\newcommand{\sm}{\bm{s}}
\newcommand{\zm}{\bm{z}}
\newcommand{\um}{\bm{u}}
\newcommand{\vm}{\bm{v}}

\newcommand{\Am}{\bm{A}}
\newcommand{\Bm}{\bm{B}}
\newcommand{\Dm}{D}
\newcommand{\Hm}{\bm{H}}
\newcommand{\Imm}{\bm{I}}
\newcommand{\Gm}{\bm{G}}

\newcommand{\Oc}[1]{\mathcal{O}\left(#1\right)}
\newcommand{\Ocs}[1]{\mathcal{O}\big(#1\big)}
\newcommand{\R}{\mathbb{R}}
\newcommand{\X}{\bm{\mathcal{X}}}
\newcommand{\W}{\mathcal{W}}
\newcommand{\Om}{\mathcal{O}}
\newcommand{\BB}{\mathcal{B}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\EEi}[1]{\mathbb{E}(#1)}
\newcommand{\Pro}{\mathbb{P}}
\newcommand{\PPi}[1]{\mathbb{P}(#1)}


\newcommand{\norm}[1]{\left\|#1\right\|}


==> sections/junks.tex <==


\subsection{Citations within the text}

Citations within the text should be based on the \texttt{natbib} package
and include the authors' last names and year (with the ``et~al.'' construct
for more than two authors). When the authors or the publication are
included in the sentence, the citation should not be in parenthesis using \verb|\citet{}| (as
in ``See \citet{Hinton06} for more information.''). Otherwise, the citation
should be in parenthesis using \verb|\citep{}| (as in ``Deep learning shows promise to make progress
towards AI~\citep{Bengio+chapter2007}.'').

The corresponding references are to be listed in alphabetical order of
authors, in the \textsc{References} section. As to the format of the
references themselves, any style is acceptable as long as it is used
consistently.

\subsection{Footnotes}

Indicate footnotes with a number\footnote{Sample of the first footnote} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches
(12~picas).\footnote{Sample of the second footnote}

\subsection{Figures}

All artwork must be neat, clean, and legible. Lines should be dark
enough for purposes of reproduction; art work should not be
hand-drawn. The figure number and caption always appear after the
figure. Place one line space before the figure caption, and one line
space after the figure. The figure caption is lower case (except for
first word and proper nouns); figures are numbered consecutively.

Make sure the figure caption does not get separated from the figure.
Leave sufficient space to avoid splitting the figure and figure caption.

You may use color figures.
However, it is best for the
figure captions and the paper body to make sense if the paper is printed
either in black/white or in color.
\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
\end{center}
\caption{Sample figure caption.}
\end{figure}

\subsection{Tables}

All tables must be centered, neat, clean and legible. Do not use hand-drawn
tables. The table number and title always appear before the table. See
Table~\ref{sample-table}.

Place one line space before the table title, one line space after the table
title, and one line space after the table. The table title must be lower case
(except for first word and proper nouns); tables are numbered consecutively.

\begin{table}[t]
\caption{Sample table title}
\label{sample-table}
\begin{center}
\begin{tabular}{ll}
\multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION}
\\ \hline \\
Dendrite         &Input terminal \\
Axon             &Output terminal \\
Soma             &Cell body (contains cell nucleus) \\
\end{tabular}
\end{center}
\end{table}

\section{Default Notation}

In an attempt to encourage standardized notation, we have included the
notation file from the textbook, \textit{Deep Learning}
\cite{goodfellow2016deep} available at
\url{https://github.com/goodfeli/dlbook_notation/}.  Use of this style
is not required and can be disabled by commenting out
\texttt{math\_commands.tex}.


\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}



\section{Final instructions}
Do not change any aspects of the formatting parameters in the style files.
In particular, do not modify the width or length of the rectangle the text
should fit into, and do not change font sizes (except perhaps in the
\textsc{References} section; see below). Please note that pages should be
numbered.

\section{Preparing PostScript or PDF files}

Please prepare PostScript or PDF files with paper size ``US Letter'', and
not, for example, ``A4''. The -t
letter option on dvips will produce US Letter files.

Consider directly generating PDF files using \verb+pdflatex+
(especially if you are a MiKTeX user).
PDF figures must be substituted for EPS figures, however.

Otherwise, please generate your PostScript and PDF files with the following commands:
\begin{verbatim}
dvips mypaper.dvi -t letter -Ppdf -G0 -o mypaper.ps
ps2pdf mypaper.ps mypaper.pdf
\end{verbatim}

\subsection{Margins in LaTeX}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+
from the graphicx package. Always specify the figure width as a multiple of
the line width as in the example below using .eps graphics
\begin{verbatim}
   \usepackage[dvips]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.eps}
\end{verbatim}
or % Apr 2009 addition
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
for .pdf graphics.
See section~4.4 in the graphics bundle documentation (\url{http://www.ctan.org/tex-archive/macros/latex/required/graphics/grfguide.ps})

A number of width problems arise when LaTeX cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command.

